Symbol Synchronization for Diffusion-Based Molecular Communications

Symbol synchronization refers to the estimation of the start of a symbol interval and is needed for reliable detection. In this paper, we develop several symbol synchronization schemes for molecular communication (MC) systems where we consider some practical challenges which have not been addressed in the literature yet. In particular, we take into account that in MC systems, the transmitter may not be equipped with an internal clock and may not be able to emit molecules with a fixed release frequency. Such restrictions hold for practical nanotransmitters, e.g. modified cells, where the lengths of the symbol intervals may vary due to the inherent randomness in the availability of food and energy for molecule generation, the process for molecule production, and the release process. To address this issue, we develop two synchronization-detection frameworks which both employ two types of molecule. In the first framework, one type of molecule is used for symbol synchronization and the other one is used for data detection, whereas in the second framework, both types of molecule are used for joint symbol synchronization and data detection. For both frameworks, we first derive the optimal maximum likelihood (ML) symbol synchronization schemes as performance upper bounds. Since ML synchronization entails high complexity, for each framework, we also propose three low-complexity suboptimal schemes, namely a linear filter-based scheme, a peak observation-based scheme, and a threshold-trigger scheme which are suitable for MC systems with limited computational capabilities. Furthermore, we study the relative complexity and the constraints associated with the proposed schemes and the impact of the insertion and deletion errors that arise due to imperfect synchronization.

==> Fig/BER_Beta/BER_Beta.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{026}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{027}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{028}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{029}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{030}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{031}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{032}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{033}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{034}[bc][bc]{\matlabtextB b)}%
\psfrag{035}[bc][bc]{\matlabtextB BER}%
\psfrag{036}[tc][tc]{\matlabtextB $\beta$}%
\psfrag{037}[bc][bc]{\matlabtextB a)}%
\psfrag{038}[bc][bc]{\matlabtextB BER}%
\psfrag{039}[tc][tc]{\matlabtextB $\beta$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.3$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.5$}%
\psfrag{005}[ct][ct]{\matlabtextB $0.6$}%
\psfrag{006}[ct][ct]{\matlabtextB $0.7$}%
\psfrag{007}[ct][ct]{\matlabtextB $0.8$}%
\psfrag{014}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{015}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{016}[ct][ct]{\matlabtextB $0.3$}%
\psfrag{017}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{018}[ct][ct]{\matlabtextB $0.5$}%
\psfrag{019}[ct][ct]{\matlabtextB $0.6$}%
\psfrag{020}[ct][ct]{\matlabtextB $0.7$}%
\psfrag{021}[ct][ct]{\matlabtextB $0.8$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextB $10^{-5}$}%
\psfrag{009}[rc][rc]{\matlabtextB $10^{-4}$}%
\psfrag{010}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{011}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{012}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{013}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{022}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{023}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{024}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{025}[rc][rc]{\matlabtextB $10^{0}$}%
%
%% </ytick>

==> Fig/BER_SNR/BER_SNR.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{025}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{026}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{027}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{028}[cl][cl]{\matlabtextA Ideal Sync., Fram. 2}%
\psfrag{029}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{030}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{031}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{032}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
\psfrag{033}[cl][cl]{\matlabtextA Ideal Sync., Fram. 1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{034}[bc][bc]{\matlabtextB b)}%
\psfrag{035}[bc][bc]{\matlabtextB BER}%
\psfrag{036}[tc][tc]{\matlabtextB SNR (dB)}%
\psfrag{037}[bc][bc]{\matlabtextB a)}%
\psfrag{038}[bc][bc]{\matlabtextB BER}%
\psfrag{039}[tc][tc]{\matlabtextB SNR (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 4$}%
\psfrag{001}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{002}[ct][ct]{\matlabtextB $0$}%
\psfrag{003}[ct][ct]{\matlabtextB $2$}%
\psfrag{004}[ct][ct]{\matlabtextB $4$}%
\psfrag{005}[ct][ct]{\matlabtextB $6$}%
\psfrag{006}[ct][ct]{\matlabtextB $8$}%
\psfrag{007}[ct][ct]{\matlabtextB $10$}%
\psfrag{012}[ct][ct]{\matlabtextB $\matlabfragNegXTick 4$}%
\psfrag{013}[ct][ct]{\matlabtextB $\matlabfragNegXTick 2$}%
\psfrag{014}[ct][ct]{\matlabtextB $0$}%
\psfrag{015}[ct][ct]{\matlabtextB $2$}%
\psfrag{016}[ct][ct]{\matlabtextB $4$}%
\psfrag{017}[ct][ct]{\matlabtextB $6$}%
\psfrag{018}[ct][ct]{\matlabtextB $8$}%
\psfrag{019}[ct][ct]{\matlabtextB $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{008}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{009}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{010}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{011}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{020}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{021}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{022}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{023}[rc][rc]{\matlabtextB $10^{0}$}%
%
%% </ytick>

==> Fig/BER_SNR_InsDel/BER_SNR_InsDel.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{007}[cl][cl]{\matlabtextA Coded TT Sync., Fram. 1}%
\psfrag{008}[cl][cl]{\matlabtextA Uncoded, TT Sync., Fram. 1}%
\psfrag{009}[cl][cl]{\matlabtextA Coded, PO. Sync., Fram. 1}%
\psfrag{010}[cl][cl]{\matlabtextA Uncoded, PO. Sync., Fram. 1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{011}[cl][cl]{\matlabtextB $\bar{T}^{\mathrm{symb}}=2$ ms}%
\psfrag{012}[cl][cl]{\matlabtextB $\bar{T}^{\mathrm{symb}}=1$ ms}%
\psfrag{013}[bc][bc]{\matlabtextB BER}%
\psfrag{014}[tc][tc]{\matlabtextB $\text{SNR}_{B}$ (dB)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextB $\matlabfragNegXTick 5$}%
\psfrag{001}[ct][ct]{\matlabtextB $0$}%
\psfrag{002}[ct][ct]{\matlabtextB $5$}%
\psfrag{003}[ct][ct]{\matlabtextB $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{005}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{-1}$}%
%
%% </ytick>

==> Fig/Concept/Concept.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{050}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{051}[cl][cl]{\matlabtextA \Tstt}%
\psfrag{052}[cl][cl]{\matlabtextA \Thr}%
\psfrag{053}[cl][cl]{\matlabtextA \B}%
\psfrag{054}[cl][cl]{\matlabtextA \A}%
\psfrag{055}[bc][bc]{\matlabtextA f) TT Sync., Fram. 2}%
\psfrag{056}[tc][tc]{\matlabtextA Time (ms)}%
\psfrag{057}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{058}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{059}[cl][cl]{\matlabtextA \Tp}%
\psfrag{060}[cl][cl]{\matlabtextA \B}%
\psfrag{061}[cl][cl]{\matlabtextA \A}%
\psfrag{062}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{063}[bc][bc]{\matlabtextA e) PO Sync., Fram. 2}%
\psfrag{064}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{065}[cl][cl]{\matlabtextA \Tlf}%
\psfrag{066}[cl][cl]{\matlabtextA \LFb}%
\psfrag{067}[cl][cl]{\matlabtextA \LFa}%
\psfrag{068}[bc][bc]{\matlabtextA d) LF Sync., Fram. 2}%
\psfrag{069}[bc][bc]{\matlabtextA Filtered Signal}%
\psfrag{070}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{071}[cl][cl]{\matlabtextA \Tml}%
\psfrag{072}[cl][cl]{\matlabtextA \MLb}%
\psfrag{073}[cl][cl]{\matlabtextA \MLa}%
\psfrag{074}[bc][bc]{\matlabtextA c) ML Sync., Fram. 2}%
\psfrag{075}[bc][bc]{\matlabtextA Log Likelihood}%
\psfrag{076}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{077}[cl][cl]{\matlabtextA \Bbar}%
\psfrag{078}[cl][cl]{\matlabtextA \B}%
\psfrag{079}[bc][bc]{\matlabtextA b) Type-$B$ Molecules, Fram. 2}%
\psfrag{080}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{081}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{082}[cl][cl]{\matlabtextA \Abar}%
\psfrag{083}[cl][cl]{\matlabtextA \A}%
\psfrag{084}[bc][bc]{\matlabtextA a) Type-$A$ Molecules, Fram. 2}%
\psfrag{085}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{086}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{087}[cl][cl]{\matlabtextA \Tett}%
\psfrag{088}[cl][cl]{\matlabtextA \Tstt}%
\psfrag{089}[cl][cl]{\matlabtextA \Thr}%
\psfrag{090}[cl][cl]{\matlabtextA \B}%
\psfrag{091}[bc][bc]{\matlabtextA f) TT Sync., Fram. 1}%
\psfrag{092}[tc][tc]{\matlabtextA Time (ms)}%
\psfrag{093}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{094}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{095}[cl][cl]{\matlabtextA \Tp}%
\psfrag{096}[cl][cl]{\matlabtextA \B}%
\psfrag{097}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{098}[bc][bc]{\matlabtextA e) PO Sync., Fram. 1}%
\psfrag{099}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{100}[cl][cl]{\matlabtextA \Tlf}%
\psfrag{101}[cl][cl]{\matlabtextA \LF}%
\psfrag{102}[bc][bc]{\matlabtextA d) LF Sync., Fram. 1}%
\psfrag{103}[bc][bc]{\matlabtextA Filtered Signal}%
\psfrag{104}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{105}[cl][cl]{\matlabtextA \Tml}%
\psfrag{106}[cl][cl]{\matlabtextA \ML}%
\psfrag{107}[bc][bc]{\matlabtextA c) ML Sync., Fram. 1}%
\psfrag{108}[bc][bc]{\matlabtextA Log Likelihood}%
\psfrag{109}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{110}[cl][cl]{\matlabtextA \Bbar}%
\psfrag{111}[cl][cl]{\matlabtextA \B}%
\psfrag{112}[bc][bc]{\matlabtextA b) Type-$B$ Molecules, Fram. 1}%
\psfrag{113}[bc][bc]{\matlabtextA $\#$ molecules}%
\psfrag{114}[cl][cl]{\matlabtextA \Tssssssss}%
\psfrag{115}[cl][cl]{\matlabtextA \Abar}%
\psfrag{116}[cl][cl]{\matlabtextA \A}%
\psfrag{117}[bc][bc]{\matlabtextA a) Type-$A$ Molecules, Fram. 1}%
\psfrag{118}[bc][bc]{\matlabtextA $\#$ molecules}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $2$}%
\psfrag{002}[ct][ct]{\matlabtextA $4$}%
\psfrag{003}[ct][ct]{\matlabtextA $6$}%
\psfrag{004}[ct][ct]{\matlabtextA $8$}%
\psfrag{005}[ct][ct]{\matlabtextA $10$}%
\psfrag{026}[ct][ct]{\matlabtextA $0$}%
\psfrag{027}[ct][ct]{\matlabtextA $2$}%
\psfrag{028}[ct][ct]{\matlabtextA $4$}%
\psfrag{029}[ct][ct]{\matlabtextA $6$}%
\psfrag{030}[ct][ct]{\matlabtextA $8$}%
\psfrag{031}[ct][ct]{\matlabtextA $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $10$}%
\psfrag{008}[rc][rc]{\matlabtextA $20$}%
\psfrag{009}[rc][rc]{\matlabtextA $0$}%
\psfrag{010}[rc][rc]{\matlabtextA $10$}%
\psfrag{011}[rc][rc]{\matlabtextA $20$}%
\psfrag{012}[rc][rc]{\matlabtextA $0$}%
\psfrag{013}[rc][rc]{\matlabtextA $5$}%
\psfrag{014}[rc][rc]{\matlabtextA $10$}%
\psfrag{015}[rc][rc]{\matlabtextA $15$}%
\psfrag{016}[rc][rc]{\matlabtextA $-250$}%
\psfrag{017}[rc][rc]{\matlabtextA $-200$}%
\psfrag{018}[rc][rc]{\matlabtextA $-150$}%
\psfrag{019}[rc][rc]{\matlabtextA $-100$}%
\psfrag{020}[rc][rc]{\matlabtextA $0$}%
\psfrag{021}[rc][rc]{\matlabtextA $10$}%
\psfrag{022}[rc][rc]{\matlabtextA $20$}%
\psfrag{023}[rc][rc]{\matlabtextA $0$}%
\psfrag{024}[rc][rc]{\matlabtextA $10$}%
\psfrag{025}[rc][rc]{\matlabtextA $20$}%
\psfrag{032}[rc][rc]{\matlabtextA $0$}%
\psfrag{033}[rc][rc]{\matlabtextA $10$}%
\psfrag{034}[rc][rc]{\matlabtextA $20$}%
\psfrag{035}[rc][rc]{\matlabtextA $0$}%
\psfrag{036}[rc][rc]{\matlabtextA $10$}%
\psfrag{037}[rc][rc]{\matlabtextA $20$}%
\psfrag{038}[rc][rc]{\matlabtextA $2000$}%
\psfrag{039}[rc][rc]{\matlabtextA $2500$}%
\psfrag{040}[rc][rc]{\matlabtextA $3000$}%
\psfrag{041}[rc][rc]{\matlabtextA $-150$}%
\psfrag{042}[rc][rc]{\matlabtextA $-100$}%
\psfrag{043}[rc][rc]{\matlabtextA $-50$}%
\psfrag{044}[rc][rc]{\matlabtextA $0$}%
\psfrag{045}[rc][rc]{\matlabtextA $10$}%
\psfrag{046}[rc][rc]{\matlabtextA $20$}%
\psfrag{047}[rc][rc]{\matlabtextA $0$}%
\psfrag{048}[rc][rc]{\matlabtextA $10$}%
\psfrag{049}[rc][rc]{\matlabtextA $20$}%
%
%% </ytick>

==> Fig/Eerror/Eerror.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{018}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{019}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{020}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{021}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{022}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{023}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{024}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{025}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
\psfrag{029}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{030}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{031}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{032}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{033}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{034}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{035}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{036}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{026}[bc][bc]{\matlabtextB b)}%
\psfrag{027}[bc][bc]{\matlabtextB $|\mathcal{E}\{\bar{e}_t[k]\}|$}%
\psfrag{028}[tc][tc]{\matlabtextB $k$}%
\psfrag{037}[bc][bc]{\matlabtextB a)}%
\psfrag{038}[bc][bc]{\matlabtextB $\mathcal{E}\{|\bar{e}_t[k]|\}$}%
\psfrag{039}[tc][tc]{\matlabtextB $k$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{009}[ct][ct]{\matlabtextB $0$}%
\psfrag{010}[ct][ct]{\matlabtextB $5$}%
\psfrag{011}[ct][ct]{\matlabtextB $10$}%
\psfrag{012}[ct][ct]{\matlabtextB $15$}%
\psfrag{013}[ct][ct]{\matlabtextB $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{014}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{015}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{016}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{017}[rc][rc]{\matlabtextB $10^{0}$}%
%
%% </ytick>

==> Fig/Eerror/RandPlot.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{022}[tc][tc]{\matlabtextA \macro}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{021}[bc][bc]{\matlabtextB random}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\bfseries\boldmath\selectfont\strut}%
\psfrag{023}[bc][bc]{\matlabtextC badness $\phi$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $1$}%
\psfrag{001}[ct][ct]{\matlabtextD $2$}%
\psfrag{002}[ct][ct]{\matlabtextD $3$}%
\psfrag{003}[ct][ct]{\matlabtextD $4$}%
\psfrag{004}[ct][ct]{\matlabtextD $5$}%
\psfrag{005}[ct][ct]{\matlabtextD $6$}%
\psfrag{006}[ct][ct]{\matlabtextD $7$}%
\psfrag{007}[ct][ct]{\matlabtextD $8$}%
\psfrag{008}[ct][ct]{\matlabtextD $9$}%
\psfrag{009}[ct][ct]{\matlabtextD $10$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextD $0$}%
\psfrag{011}[rc][rc]{\matlabtextD $0.1$}%
\psfrag{012}[rc][rc]{\matlabtextD $0.2$}%
\psfrag{013}[rc][rc]{\matlabtextD $0.3$}%
\psfrag{014}[rc][rc]{\matlabtextD $0.4$}%
\psfrag{015}[rc][rc]{\matlabtextD $0.5$}%
\psfrag{016}[rc][rc]{\matlabtextD $0.6$}%
\psfrag{017}[rc][rc]{\matlabtextD $0.7$}%
\psfrag{018}[rc][rc]{\matlabtextD $0.8$}%
\psfrag{019}[rc][rc]{\matlabtextD $0.9$}%
\psfrag{020}[rc][rc]{\matlabtextD $1$}%
%
%% </ytick>

==> Fig/Error_ISI/Error_ISI.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{023}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{024}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{025}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{026}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{027}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{028}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{029}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{030}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
\psfrag{034}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{035}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{036}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{037}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{038}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{039}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{040}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{041}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{031}[bc][bc]{\matlabtextB b)}%
\psfrag{032}[bc][bc]{\matlabtextB $\mathcal{E}\{|\bar{e}_t[k]|\}$}%
\psfrag{033}[tc][tc]{\matlabtextB $\bar{T}^{\mathrm{symb}}$ (ms)}%
\psfrag{042}[bc][bc]{\matlabtextB a)}%
\psfrag{043}[bc][bc]{\matlabtextB $\mathcal{E}\{|\bar{e}_t[k]|\}$}%
\psfrag{044}[tc][tc]{\matlabtextB $\alpha$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextB $0.5$}%
\psfrag{001}[ct][ct]{\matlabtextB $1$}%
\psfrag{002}[ct][ct]{\matlabtextB $1.5$}%
\psfrag{003}[ct][ct]{\matlabtextB $2$}%
\psfrag{004}[ct][ct]{\matlabtextB $2.5$}%
\psfrag{005}[ct][ct]{\matlabtextB $3$}%
\psfrag{011}[ct][ct]{\matlabtextB $0.1$}%
\psfrag{012}[ct][ct]{\matlabtextB $0.15$}%
\psfrag{013}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{014}[ct][ct]{\matlabtextB $0.25$}%
\psfrag{015}[ct][ct]{\matlabtextB $0.3$}%
\psfrag{016}[ct][ct]{\matlabtextB $0.35$}%
\psfrag{017}[ct][ct]{\matlabtextB $0.4$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{009}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{010}[rc][rc]{\matlabtextB $10^{1}$}%
\psfrag{018}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{019}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{020}[rc][rc]{\matlabtextB $10^{-1}$}%
\psfrag{021}[rc][rc]{\matlabtextB $10^{0}$}%
\psfrag{022}[rc][rc]{\matlabtextB $10^{1}$}%
%
%% </ytick>

==> Fig/InsDel/InsDel.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{019}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{020}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{021}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{022}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{023}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{024}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{025}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{026}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
\psfrag{030}[cl][cl]{\matlabtextA TT Sync., Fram. 2}%
\psfrag{031}[cl][cl]{\matlabtextA PO Sync., Fram. 2}%
\psfrag{032}[cl][cl]{\matlabtextA LF Sync., Fram. 2}%
\psfrag{033}[cl][cl]{\matlabtextA ML Sync., Fram. 2}%
\psfrag{034}[cl][cl]{\matlabtextA TT Sync., Fram. 1}%
\psfrag{035}[cl][cl]{\matlabtextA PO Sync., Fram. 1}%
\psfrag{036}[cl][cl]{\matlabtextA LF Sync., Fram. 1}%
\psfrag{037}[cl][cl]{\matlabtextA ML Sync., Fram. 1}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{027}[bc][bc]{\matlabtextB b)}%
\psfrag{028}[bc][bc]{\matlabtextB Deletion Error Probability}%
\psfrag{029}[tc][tc]{\matlabtextB $k$}%
\psfrag{038}[bc][bc]{\matlabtextB a)}%
\psfrag{039}[bc][bc]{\matlabtextB Insertion Error Probability}%
\psfrag{040}[tc][tc]{\matlabtextB $k$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $5$}%
\psfrag{002}[ct][ct]{\matlabtextB $10$}%
\psfrag{003}[ct][ct]{\matlabtextB $15$}%
\psfrag{004}[ct][ct]{\matlabtextB $20$}%
\psfrag{009}[ct][ct]{\matlabtextB $0$}%
\psfrag{010}[ct][ct]{\matlabtextB $5$}%
\psfrag{011}[ct][ct]{\matlabtextB $10$}%
\psfrag{012}[ct][ct]{\matlabtextB $15$}%
\psfrag{013}[ct][ct]{\matlabtextB $20$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextB $10^{-5}$}%
\psfrag{006}[rc][rc]{\matlabtextB $10^{-4}$}%
\psfrag{007}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{008}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{014}[rc][rc]{\matlabtextB $10^{-5}$}%
\psfrag{015}[rc][rc]{\matlabtextB $10^{-4}$}%
\psfrag{016}[rc][rc]{\matlabtextB $10^{-3}$}%
\psfrag{017}[rc][rc]{\matlabtextB $10^{-2}$}%
\psfrag{018}[rc][rc]{\matlabtextB $10^{-1}$}%
%
%% </ytick>

==> Fig/PDFerror/PDFerror.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{024}[cl][cl]{\matlabtextA TT Sync.}%
\psfrag{025}[cl][cl]{\matlabtextA PO Sync.}%
\psfrag{026}[cl][cl]{\matlabtextA LF Sync.}%
\psfrag{027}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{028}[bc][bc]{\matlabtextA b) Synchronization Framework 2}%
\psfrag{029}[bc][bc]{\matlabtextA PDF}%
\psfrag{030}[tc][tc]{\matlabtextA Normalized Synchronization Error, $\bar{e}_t[k]$}%
\psfrag{031}[cl][cl]{\matlabtextA TT Sync.}%
\psfrag{032}[cl][cl]{\matlabtextA PO Sync.}%
\psfrag{033}[cl][cl]{\matlabtextA LF Sync.}%
\psfrag{034}[cl][cl]{\matlabtextA ML Sync.}%
\psfrag{035}[bc][bc]{\matlabtextA a) Synchronization Framework 1}%
\psfrag{036}[bc][bc]{\matlabtextA PDF}%
\psfrag{037}[tc][tc]{\matlabtextA Normalized Synchronization Error, $\bar{e}_t[k]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $\matlabfragNegXTick 2$}%
\psfrag{001}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1$}%
\psfrag{002}[ct][ct]{\matlabtextA $0$}%
\psfrag{003}[ct][ct]{\matlabtextA $1$}%
\psfrag{004}[ct][ct]{\matlabtextA $2$}%
\psfrag{012}[ct][ct]{\matlabtextA $\matlabfragNegXTick 2$}%
\psfrag{013}[ct][ct]{\matlabtextA $\matlabfragNegXTick 1$}%
\psfrag{014}[ct][ct]{\matlabtextA $0$}%
\psfrag{015}[ct][ct]{\matlabtextA $1$}%
\psfrag{016}[ct][ct]{\matlabtextA $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{005}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{006}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{007}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{008}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{009}[rc][rc]{\matlabtextA $10^{0}$}%
\psfrag{010}[rc][rc]{\matlabtextA $10^{1}$}%
\psfrag{011}[rc][rc]{\matlabtextA $10^{2}$}%
\psfrag{017}[rc][rc]{\matlabtextA $10^{-4}$}%
\psfrag{018}[rc][rc]{\matlabtextA $10^{-3}$}%
\psfrag{019}[rc][rc]{\matlabtextA $10^{-2}$}%
\psfrag{020}[rc][rc]{\matlabtextA $10^{-1}$}%
\psfrag{021}[rc][rc]{\matlabtextA $10^{0}$}%
\psfrag{022}[rc][rc]{\matlabtextA $10^{1}$}%
\psfrag{023}[rc][rc]{\matlabtextA $10^{2}$}%
%
%% </ytick>
